Evidential Uncertainty Probes for Graph Neural Networks

Accurate quantification of both aleatoric and epistemic uncertainties is essential when deploying Graph Neural Networks (GNNs) in high-stakes applications such as drug discovery and financial fraud detection, where reliable predictions are critical. Although Evidential Deep Learning (EDL) efficiently quantifies uncertainty using a Dirichlet distribution over predictive probabilities, existing EDL-based GNN (EGNN) models require modifications to the network architecture and retraining, failing to take advantage of pre-trained models. We propose a plug-and-play framework for uncertainty quantification in GNNs that works with pre-trained models without the need for retraining. Our Evidential Probing Network (EPN) uses a lightweight Multi-Layer-Perceptron (MLP) head to extract evidence from learned representations, allowing efficient integration with various GNN architectures. We further introduce evidence-based regularization techniques, referred to as EPN-reg, to enhance the estimation of epistemic uncertainty with theoretical justifications. Extensive experiments demonstrate that the proposed EPN-reg achieves state-of-the-art performance in accurate and efficient uncertainty quantification, making it suitable for real-world deployment.

==> discussion.tex <==
Next, we use a standard result about Gaussian random variables. If $k$ is distributed as $ \mathcal{N}(m, s^2)$, then there exists a standard normal variable $ \xi \sim \mathcal{N}(0,1) $ such that
\begin{equation}
  k = m + s\xi.  
\end{equation}

Thus, for any function $f(\cdot)$ for which the expectation exists, we have
\begin{equation}
    \mathbb{E}_{k \sim \mathcal{N}(m,s^2)} \left[ f(k) \right] = \mathbb{E}_{\xi \sim \mathcal{N}(0,1)} \left[ f(m + s\xi) \right].
\end{equation}

Choosing $ f(k) = \upsilon(\cosh(k)) $ we obtain
\begin{equation}
\begin{aligned}
       L(\mathbf{w}_P, b_P) &= \mathbb{E}_{\xi \sim \mathcal{N}(0,1)} \left[ \upsilon (\cosh(m + s\xi)) \right]. \\
m&=\mathbf{w}_P \boldsymbol{\mu} + b_P, \quad s^2 = \mathbf{w}_P\boldsymbol{\Sigma}\mathbf{w}^\top_P
\end{aligned}
\end{equation}

Suppose we scale the parameters by a positive constant $t > 0$. That is, define
    \begin{equation}
        \mathbf{w}_P' = t \mathbf{w}_P, \quad b_P' = t b_P.
    \end{equation}
    Then
    \begin{equation}
        m' = t m, \quad s' = t s.
    \end{equation}
 With these new parameters, the loss becomes
    \begin{equation}
        L(\mathbf{w}_P', b_P') = \mathbb{E}_{\xi \sim \mathcal{N}(0,1)} \left[ \upsilon (\cosh (t(m + s\xi))) \right].
    \end{equation}
    
Since the function $\cosh(\cdot)$ grows (roughly exponentially) for large value and $\upsilon (\cdot) $ is monotonically decreasing, increasing the scale $t$ makes the argument $t(m + s\xi) $ larger in absolute value for almost all $ \xi $. This in turn makes $ \cosh(t(m + s\xi)) $ larger, and because $ \upsilon(\cdot) $ is decreasing, the overall loss becomes smaller. In other words, by increasing $ t $, one can always reduce the loss.

Thus, if no constraint is placed on the norm of  $\mathbf{w}_P $ (or on $ b_P $), the minimization is degenerate: one may lower the loss arbitrarily by taking $ t \to \infty $. The optimum is only reached in the limit
    \begin{equation}
        \|\mathbf{w}_P\| \to \infty \quad \text{or} \quad |b_P| \to \infty.
    \end{equation}
{\color{red} Linlin: How to verify the `or'}

\textbf{Step 2: give an example of optimal solution}

Considering one optimum solution that 
\begin{equation}
\begin{aligned}
    \mathbf{w}_P^* &= t^* \mathbf{w}_0, \quad b_p^* = t^* b_0, \\ 
    \mathbf{w}_0 &= \textbf{0}, \quad b_0 = \frac{1}{\epsilon}, \quad  t^* \to \infty
\end{aligned}
\end{equation}
\textbf{Step 3: Prove that probability is less than $\epsilon$}
 
Then we prove that 
\begin{equation}
        \mathbb{P}\bigr(U^*(\mathbf{z}_0)> U^*(\mathbf{z_{1}})\bigr)<\epsilon, \forall \mathbf{z}_0\sim \mathcal{N}(\textbf{0}, \boldsymbol{\Sigma}), \mathbf{z}_{1}\sim \mathcal{N}(\bm{\mu}, \boldsymbol{\Sigma}).
\end{equation}
where 
\begin{equation}
\begin{aligned}
       U^*(\mathbf{z}_0) &= \frac{2}{\,\cosh \bigl(\mathbf{w}_P^* \mathbf{z}_0 + b_P^*\bigr) + 2\,} \quad \mathbf{z}_0\sim \mathcal{N}(\textbf{0}, \boldsymbol{\Sigma}) \\
    U^*(\mathbf{z}_1) &= \frac{2}{\,\cosh \bigl(\mathbf{w}_P^* \mathbf{z}_1 + b_P^*\bigr) + 2\,} \quad \mathbf{z}_{1}\sim \mathcal{N}(\bm{\mu}, \boldsymbol{\Sigma})  
\end{aligned}
\end{equation}

Therefore,
\begin{equation}
\begin{aligned}
        \mathbb{P}\bigl(U^*(\mathbf{z}_0)> U^*(\mathbf{z_{1}})\bigr) &= \mathbb{P}\bigl( |\mathbf{w}_P^* \mathbf{z}_0 + b_P^*| < |\mathbf{w}_P^* \mathbf{z}_1 + b_P^*|\bigr) \\
        &= \mathbb{P}\bigl( |\mathbf{w}_0 \mathbf{z}_0 + b_0| < |\mathbf{w}_0 \mathbf{z}_1 + b_0|\bigr) 
\end{aligned}
\end{equation}
Replace the $\mathbf{w}_0, b_0$, then we have
\begin{equation}
    \begin{aligned}
        \mathbb{P}\bigl(U^*(\mathbf{z}_0)> U^*(\mathbf{z_{1}})\bigr) 
        &= \mathbb{P}\bigl( |b_0| < |b_0|\bigr) \\
        &= 0
    \end{aligned}
\end{equation}

